DIVINE: Diverse Influential Training Points for Data Visualization and Model Refinement

As the complexity of machine learning (ML) models increases, resulting in a lack of prediction explainability, several methods have been developed to explain a model's behavior in terms of the training data points that most influence the model. However, these methods tend to mark outliers as highly influential points, limiting the insights that practitioners can draw from points that are not representative of the training data. In this work, we take a step towards finding influential training points that also represent the training data well. We first review methods for assigning importance scores to training points. Given importance scores, we propose a method to select a set of DIVerse INfluEntial (DIVINE) training points as a useful explanation of model behavior. As practitioners might not only be interested in finding data points influential with respect to model accuracy, but also with respect to other important metrics, we show how to evaluate training data points on the basis of group fairness. Our method can identify unfairness-inducing training points, which can be removed to improve fairness outcomes. Our quantitative experiments and user studies show that visualizing DIVINE points helps practitioners understand and explain model behavior better than earlier approaches.

==> additional_Eval.tex <==
We report additional evaluation functions $f$ that can be used to score data points in Table~\ref{tab:eval}.  For every evaluation function, we write the function such that a large $f(\theta)$ is undesirable: a negative importance score (if $g$ is taken to be the difference between $f$ evaluated at the new and old parameters -- trained with and without the point respectively) implies that a point is harmful to $f$. Moreover, definitions of $g$ that are independent of $f$ are also possible, e.g.,
$g(\theta_{\text{new}}, \theta_{\text{old}}) = ||\theta_{\text{new}} - \theta_{\text{old}}||_p$.
However, from a model debugging perspective, these definitions may not be relevant when the dimensionality of $\theta$ is even moderately large.
\begin{table*}[htb]
\centering
\begin{tabular}{l|l}
\toprule
                Metric    &  Evaluation Function ($f$) \\ 
\midrule

Loss (e.g., wrt $\mathcal{D}_\text{train}$) & $f_{\text{train}}(\theta) = \mathcal{L}(\mathcal{D}_\text{train}) = \sum_{i}^{n} l(x_i,y_i; \theta)$ \\
\midrule
Eq. Accuracy~\citep{berk2018fairness} & $f_\text{ea}(\theta) = f_\text{unf}(\theta) = \sum_{j \in \{-1,1\}} |P(\hat y = j |A = a, y = j) - P(\hat y = j |A = b, y = j)|$ \\
\midrule
Eq. Opportunity~\citep{hardt2016} & $f_\text{eq}(\theta) =  P(\hat y = 1 |A = a, y = 1) - P(\hat y = 1 |A = b, y = 1)$ \\
\midrule
Eq. Odds~\citep{hardt2016} & $f_\text{eo}(\theta) =  \sum_{j \in \{-1,1\}}  |P(\hat y = 1 |A = a, y = j) - P(\hat y = 1 |A = b, y = j)|$ \\
% \midrule
% Robustness & $f_\text{r}(\theta) = $ \\ \midrule
% Covariate Shift & $f_\text{cs}(\theta) = $ \\ \midrule
% Label Shift & $f_\text{ls}(\theta) = $ \\ 
\bottomrule
\end{tabular}
\caption{Various candidate evaluation functions $f$.}
\label{tab:eval}
\end{table*}
% Moreover, we can re-write our definition of unfairness from the main paper (as well as other fairness metrics from Table~\ref{tab:eval}) in terms of the model's loss, $\mathcal{L}(\cdot)$.
% \begin{enumerate}
%     \item Equal Opportunity (EQ): Parameters $\theta$ are considered to be fair wrt EQ if the following quantity is close to 0:  
%     % $$P(\hat y = 1 |a = 0, y = 1) - P(\hat y = 1 |a = 1, y = 1)$$ 
%     $$ f_{\text{ap-eq}}(\theta) = \mathcal{L}(\mathcal{D}_{+a+}) - \mathcal{L}(\mathcal{D}_{+b+})$$ 
%     That is, the true positive rates for both groups should the same~\citep{hardt2016equality}.
%     \item Equal Accuracy (EA): Parameters $\theta$ are considered to be fair wrt EA if the following quantity is close to 0:
%     % $$ \sum_{j \in \{0,1\}} |P(\hat y = j |a = 0, y = j) - P(\hat y = j |a = 1, y = j)|
%     % $$ 
%     % $$ f_{\text{ea}}(\theta) = |\mathcal{L}(\mathcal{D}_{-a-}) - \mathcal{L}(\mathcal{D}_{-b-}) | + |\mathcal{L}(\mathcal{D}_{+a+}) - \mathcal{L}(\mathcal{D}_{+b+})|$$ 
%     % $$ f_{\text{ea}}(\theta) = |\mathcal{L}(\mathcal{D}_{-a-}) - \mathcal{L}(\mathcal{D}_{-b-}) | + |f_{\text{eq}}(\theta)|$$ 
%     $$ f_{\text{ap-unf}}(\theta) = f_{\text{ap-ea}}(\theta) = \mathcal{L}(\mathcal{D}_{a}) - \mathcal{L}(\mathcal{D}_{b})$$ 
%     That is, the classifier accuracy for both groups should be the same~\citep{berk2018fairness}.
%     \item Equalized Odds (EO): Parameters $\theta$ are considered to be fair wrt EO if the following quantity is close to 0:  
%     % $$ |P(\hat Y = 1 |A = 0, Y = 0) - P(\hat Y = 1 |A = 1, Y = 0)| +|P(\hat Y = 1 |A = 0, Y = 1) - P(\hat Y = 1 |A = 1, Y = 1)| $$ 
%     % $$ \sum_{j \in \{0,1\}} |P(\hat y = 1 |a = 0, y = j) - P(\hat y = 1 |a = 1, y = j)|
%     % $$ 
%     % $$ f_{\text{eo}}(\theta) = |\mathcal{L}(\mathcal{D}_{-a+}) - \mathcal{L}(\mathcal{D}_{-b+}) | + |\mathcal{L}(\mathcal{D}_{+a+}) - \mathcal{L}(\mathcal{D}_{+b+})|$$ 
%     $$ f_{\text{ap-eo}}(\theta) = |\mathcal{L}(\mathcal{D}_{-a+}) - \mathcal{L}(\mathcal{D}_{-b+}) | + |f_{\text{ap-eq}}(\theta)|$$ 
%     That is, we want to equalize the true positive and false positive rates across groups~\citep{hardt2016equality}. EO is satisfied if $\hat{y}$ and ${A}$ are independent conditional on $y$.
% \end{enumerate}
% Note $f_{\text{train}}(\theta) = \mathcal{L}(\mathcal{D})$. 
We can also define importance scores that jointly consider unfairness and loss: $f(\theta) = f_{\text{train}}(\theta) + f_{\text{unf}}(\theta)$ would tell us how important a point is for unfairness and loss. 

% We can consider approximating unfairness (Equation~\ref{eq:ea}) in terms of the model's loss, $\mathcal{L}(\cdot)$, as follows: $$f_{\text{ap-unf}}(\theta) = \frac{1}{|\mathcal{D}_{a}|}\mathcal{L}(\mathcal{D}_{a}) - \frac{1}{|\mathcal{D}_{b}|}\mathcal{L}(\mathcal{D}_{b})$$
% Since $f_{\text{unf}}$ can be written as a sum of loss terms and our loss is assumed to be twice differentiable and continuous, we can write the influence on dropping a training point on $f_{\text{unf}}$ using Equation~\ref{generic}. Note that: \begin{equation*}
% \small
%     \nabla_{\theta} f_{\text{ap-unf}}(\hat \theta) = \sum_{j \in D_{a}} \frac{\nabla_{\theta}l(x_j,y_j; \hat \theta)}{|\mathcal{D}_{a}|}- \sum_{k \in D_{b}}\frac{\nabla_{\theta}l(x_k,y_k; \hat \theta)}{|\mathcal{D}_{b}|}
% \end{equation*}. With some  rearrangement, we get the following:
% \begin{equation}
% \small
%     I_i^{f_{\text{ap-unf}}} = \nabla_{\theta} \; l(x_i,y_i; \hat \theta)^\intercal \left[ \sum_{j \in \mathcal{D}} \psi_j H_{\hat \theta}^{-1}\nabla_{\theta} \; l(x_j,y_j; \hat \theta) \right]
%     \label{inf_eq}
% \end{equation}
% where $\psi_j$ is $\frac{1}{|\mathcal{D}_{b}|}$ if $j \in \mathcal{D}_{b}$, $\frac{-1}{|\mathcal{D}_{a}|}$ if $j \in \mathcal{D}_{a}$, and zero otherwise. Such approximate influence methods may be helpful to practitioners dealing with large datasets and large non-convex models.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See the second paragraph of Section~\ref{conc}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our paper focuses on providing transparency into ML models. Many have noted that transparency mechanisms can be gamed to provide an illusion of safety ~\citep{weller2019transparency}. Specifically, some have shown that deceptive explanations can be generated from popular explainability methods~\citep{dimanov2020you,slack2020fooling}. Gamed explanations might lead stakeholders to misplace trust~\citep{lakkaraju2020fool}. We acknowledge that similar gaming of explanations is likely plausible with training point importance, leading practitioners to believe that some points have more influence than they actually do.
    %to be a potential negative societal impact of our work. In future work, we must examine the robustness of DIVINE to providing deceptive data points that may intentionally mislead a practitioner. 
    }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Appendix~\ref{guide}. We include a detailed guide into parameter selection in addition to descriptions (including code snippets) of use cases for our DIVINE codebase. In the codebase itself, we provide a detailed README regarding code functionality.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{app:setup}. We describe how hyperparameters were selected and how data was generated and refined for experimentation. Additionally, this is all replicable from our codebase.}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section~\ref{user_study}. We reported error bars for there results of our user studies. Results for Section~\ref{experiments} were run with a fixed random seed, enabling reproducibility.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Experiments were all run on local machines, using CPUs only. }
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{experiments}, where we introduce and cite the publicly available datasets we used for our experiments.}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix~\ref{app:setup}, which describes the publicly available datasets we used for our experiments.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Appendix~\ref{hse} for a description of how our user studies were set up and for figures shown to participants.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{See Appendix~\ref{hse}.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See Section~\ref{hse}.}
\end{enumerate}

\end{enumerate}
